Generic Camera Attribute Control using Bayesian Optimization

Cameras are the most widely exploited sensor in both robotics and computer vision communities. Despite their popularity, two dominant attributes (i.e., gain and exposure time) have been determined empirically and images are captured in very passive manner. In this paper, we present an active and generic camera attribute control scheme using Bayesian optimization. We extend from our previous work [1] in two aspects. First, we propose a method that jointly controls camera gain and exposure time. Secondly, to speed up the Bayesian optimization process, we introduce image synthesis using the camera response function (CRF). These synthesized images allowed us to diminish the image acquisition time during the Bayesian optimization phase, substantially improving overall control performance. The proposed method is validated both in an indoor and an outdoor environment where light condition rapidly changes. Supplementary material is available at https://youtu.be/XTYR_Mih3OU .

==> fig_ctrl.tex <==
\begin{figure*}[!t]
  \centering%
  \def\width{0.29\columnwidth}%

  \begin{minipage}[b]{0.49\textwidth}%
  \centering%
    % -------------- SUBFIGURE -1 -------------- %
    \subfigure[ACQ 1]{
    \includegraphics[width=\width] {./figs/ctrl/acq_1}
    \label{fig:acq1}
  }
    % -------------- SUBFIGURE -2 -------------- %
    \subfigure[ACQ 2]{
    \includegraphics[width=\width] {./figs/ctrl/acq_2}
    \label{fig:acq2}
  }
    % -------------- SUBFIGURE -3 -------------- %
    \subfigure[ACQ 3]{
    \includegraphics[width=\width] {./figs/ctrl/acq_3}
    \label{fig:acq3}
  }
  \\
    % -------------- SUBFIGURE -4 -------------- %
    \subfigure[ACQ 4]{
    \includegraphics[width=\width] {./figs/ctrl/acq_4}
    \label{fig:acq4}
  }
    % -------------- SUBFIGURE -5 -------------- %
    \subfigure[ACQ 5]{
    \includegraphics[width=\width] {./figs/ctrl/acq_5}
    \label{fig:acq5}
  }
    % -------------- SUBFIGURE -6 -------------- %
    \subfigure[ACQ 8]{
    \includegraphics[width=\width] {./figs/ctrl/acq_8}
    \label{fig:acq6}
  }
  \end{minipage}%
  \begin{minipage}[b]{0.45\textwidth}%
  \centering%
    % -------------- SUBFIGURE -1 -------------- %
    \subfigure[MET 1]{
    \includegraphics[width=\width] {./figs/ctrl/met_1}
    \label{fig:met1}
  }
    % -------------- SUBFIGURE -2 -------------- %
    \subfigure[MET 2]{
    \includegraphics[width=\width] {./figs/ctrl/met_2}
    \label{fig:met2}
  }
    % -------------- SUBFIGURE -3 -------------- %
    \subfigure[MET 3]{
    \includegraphics[width=\width] {./figs/ctrl/met_3}
    \label{fig:met3}
  }
  \\
    % -------------- SUBFIGURE -4 -------------- %
    \subfigure[MET 4]{
    \includegraphics[width=\width] {./figs/ctrl/met_4}
    \label{fig:met4}
  }
    % -------------- SUBFIGURE -5 -------------- %
    \subfigure[MET 5]{
    \includegraphics[width=\width] {./figs/ctrl/met_5}
    \label{fig:met5}
  }
    % -------------- SUBFIGURE -6 -------------- %
    \subfigure[MET 6]{
    \includegraphics[width=\width] {./figs/ctrl/met_8}
    \label{fig:met8}
  }
  \end{minipage}

  \caption{\hl{CHO: please add caption}} 
    
  \label{fig:ctrl}
\end{figure*}


==> fig_metric_eval.tex <==
%\begin{figure*}[!t]
%  \centering%
%  \def\width{0.25\columnwidth}%
%  \centering%
%    % -------------- SUBFIGURE -1 -------------- %
%    \subfigure[10]{
%	\includegraphics[trim = 30 280 170 250, clip, width=\width]{./figs/env_lux/3d7_18}% l b r t
%    \label{fig:env1}
%  }
%    % -------------- SUBFIGURE -2 -------------- %
%    \subfigure[50]{
%	\includegraphics[trim = 30 280 170 250, clip, width=\width] {./figs/env_lux/3d43}
%    \label{fig:env2}
%  }
%    % -------------- SUBFIGURE -3 -------------- %
%    \subfigure[80]{
%	\includegraphics[trim = 30 280 170 250, clip, width=\width] {./figs/env_lux/3d86}
%    \label{fig:env3}
%  }
%    % -------------- SUBFIGURE -4 -------------- %
%    \subfigure[100]{
%	\includegraphics[trim = 30 280 170 250, clip, width=\width] {./figs/env_lux/3d110}
%    \label{fig:env4}
%  }
%    % -------------- SUBFIGURE -5 -------------- %
%    \subfigure[320]{
%	\includegraphics[trim = 30 280 170 250, clip, width=\width] {./figs/env_lux/3d344}
%    \label{fig:env5}
%  }
%    % -------------- SUBFIGURE -6 -------------- %
%    \subfigure[400]{
%	\includegraphics[trim = 30 280 170 250, clip, width=\width] {./figs/env_lux/3d458}
%    \label{fig:env6}
%  }
%    % -------------- SUBFIGURE -7 -------------- %
%    \subfigure[1000]{
%	\includegraphics[trim = 30 280 170 250, clip, width=\width] {./figs/env_lux/3d750}
%    \label{fig:env7}
%  }  \\
%    % -------------- SUBFIGURE -1 -------------- %
%     \subfigure[10]{
% 	\includegraphics[trim = 30 280 170 250, clip, width=\width]{./figs/env_lux/18g_surf}% l b r t
%     \label{fig:gain1}
%   }
%     % -------------- SUBFIGURE -2 -------------- %
%     \subfigure[50]{
% 	\includegraphics[trim = 30 280 170 250, clip, width=\width] {./figs/env_lux/43g_surf}
%     \label{fig:gain2}
%   }
%     % -------------- SUBFIGURE -3 -------------- %
%     \subfigure[80]{
% 	\includegraphics[trim = 30 280 170 250, clip, width=\width] {./figs/env_lux/86g_surf}
%     \label{fig:gain3}
%   }
%     % -------------- SUBFIGURE -4 -------------- %
%     \subfigure[100]{
% 	\includegraphics[trim = 30 280 170 250, clip, width=\width] {./figs/env_lux/110g_surf}
%     \label{fig:gain4}
%   }
%     % -------------- SUBFIGURE -5 -------------- %
%     \subfigure[320]{
% 	\includegraphics[trim = 30 280 170 250, clip, width=\width] {./figs/env_lux/344g_surf}
%     \label{fig:gain5}
%   }
%     % -------------- SUBFIGURE -6 -------------- %
%     \subfigure[400]{
% 	\includegraphics[trim = 30 280 170 250, clip, width=\width] {./figs/env_lux/458g_surf}
%     \label{fig:gain6}
%   }
%     % -------------- SUBFIGURE -7 -------------- %
%     \subfigure[1000]{
% 	\includegraphics[trim = 30 280 170 250, clip, width=\width] {./figs/env_lux/750g_surf}
%     \label{fig:gain7}
%   }  \\

%  \begin{minipage}{0.9\textwidth}
%    \small
%    \centering
%    \begin{tabular}{c|ccccccc}
%      \textbf{Illuminance {[}lux{]}}  & 10                         & 50                   & 80               & 100               & 320             & 400                & 1000\\
%      \hline
%      \textbf{environment}            & \textit{Dark surroundings} & \textit{Living room} & \textit{Hallway} & \textit{Dark day} & \textit{Office} & \textit{Sunny day} & \textit{Artificial lighting}\\
%      \hline
%      \textbf{Optimal $\Delta$t [ms]} & 17.0                       & 20.0                 & 5.5              & 5.5               &   2.5           & 2.0                & 2.0\\
%      \hline
%      \textbf{Optimal gain [dB]}      & 11                         & 3                    & 0                & 0                 &  12             & 4                  & 1\\
%      \hline\hline
%      \textbf{Optimal $\Delta$t [ms]} & 19.5                       & 12.5                 & 5.5              & 5.0               &   7.0           & 2.0                & 1.5\\
%      \hline
%      \textbf{Optimal gain [dB]}      & 9                          & 0                    & 0                & 0                 &  2              & 4                  & 0
%
%    \end{tabular}
%  \end{minipage}
%  \caption{Image evaluation metric plotted with respect to the gain and exposure time.}
%  \label{fig:metric_eval}
%\end{figure*}


==> fig_synth_exp_indoor.tex <==
\begin{figure*}[!t]
  \centering%
  \def\width{0.25\columnwidth}%
  \begin{minipage}[b]{0.49\textwidth}%
  \centering%
    % -------------- SUBFIGURE -1 -------------- %
    \subfigure[real 1ms]{
    \includegraphics[width=\width] {./figs/real/1}
    \label{fig:r1}
  }
    % -------------- SUBFIGURE -2 -------------- %
    \subfigure[real 4ms]{
    \includegraphics[width=\width] {./figs/real/4}
    \label{fig:r2}
  }
    % -------------- SUBFIGURE -3 -------------- %
    \subfigure[real 6ms]{
    \includegraphics[width=\width] {./figs/real/6}
    \label{fig:r3}
  }
  \\
    % -------------- SUBFIGURE -4 -------------- %
    \subfigure[real 8ms]{
    \includegraphics[width=\width] {./figs/real/8}
    \label{fig:r4}
  }
    % -------------- SUBFIGURE -5 -------------- %
    \subfigure[real 14ms]{
    \includegraphics[width=\width] {./figs/real/14}
    \label{fig:r7}
  }
    % -------------- SUBFIGURE -6 -------------- %
    \subfigure[real 18ms]{
    \includegraphics[width=\width] {./figs/real/18}
    \label{fig:r9}
  }
  \end{minipage}%
  \begin{minipage}[b]{0.45\textwidth}%
  \centering%
    % -------------- SUBFIGURE -1 -------------- %
    \subfigure[synthetic 1ms]{
    \includegraphics[width=\width] {./figs/synth/ss1}
    \label{fig:s1}
  }
    % -------------- SUBFIGURE -2 -------------- %
    \subfigure[synthetic 4ms]{
    \includegraphics[width=\width] {./figs/synth/ss4}
    \label{fig:s2}
  }
    % -------------- SUBFIGURE -3 -------------- %
    \subfigure[synthetic 6ms]{
    \includegraphics[width=\width] {./figs/synth/ss6}
    \label{fig:s3}
  }
  \\
    % -------------- SUBFIGURE -4 -------------- %
    \subfigure[synthetic 8ms]{
    \includegraphics[width=\width] {./figs/synth/ss8}
    \label{fig:s4}
  }
    % -------------- SUBFIGURE -5 -------------- %
    \subfigure[synthetic 14ms]{
    \includegraphics[width=\width] {./figs/synth/ss14}
    \label{fig:s7}
  }
    % -------------- SUBFIGURE -6 -------------- %
    \subfigure[synthetic 18ms]{
    \includegraphics[width=\width] {./figs/synth/ss18}
    \label{fig:s9}
  }
  \end{minipage}\\
  \begin{minipage}[b]{0.45\textwidth}%
  \centering%
    \subfigure[Optimal (4ms)]{
    \includegraphics[width=0.3\textwidth] {./figs/real/4}
    \label{fig:opt_real}
  }
    \subfigure[EWG]{
    \includegraphics[trim = 100 280 120 280, clip, width=0.3\textwidth]{./figs/EWG_real.pdf}% l b r t
    \label{fig:EWG_real}
  }
  \end{minipage}
  \begin{minipage}[b]{0.45\textwidth}%
  \centering%
    \includegraphics[width=0.3\textwidth] {./figs/synth/ss4}
    \includegraphics[trim = 100 280 120 280, clip, width=0.3\textwidth]{./figs/EWG_syn.pdf}% l b r t

  \end{minipage}

  \caption{Comparison of synthetic images and actual images along the exposure time variation.}

  \label{fig:synth_exp}
\end{figure*}


==> fig_synth_exp_outdoor.tex <==
\begin{figure*}[!t]
  \centering%
  \def\width{0.25\columnwidth}%
  \begin{minipage}[b]{0.49\textwidth}%
  \centering%
    % -------------- SUBFIGURE -1 -------------- %
    \subfigure[real 50us]{
    \includegraphics[width=\width] {./figs/real_out/1}
    \label{fig:r1_out}
  }
    % -------------- SUBFIGURE -2 -------------- %
    \subfigure[real 95us]{
    \includegraphics[width=\width] {./figs/real_out/10}
    \label{fig:r2_out}
  }
    % -------------- SUBFIGURE -3 -------------- %
    \subfigure[real 140us]{
    \includegraphics[width=\width] {./figs/real_out/20}
    \label{fig:r3_out}
  }
  \\
    % -------------- SUBFIGURE -4 -------------- %
    \subfigure[real 235us]{
    \includegraphics[width=\width] {./figs/real_out/40}
    \label{fig:r4_out}
  }
    % -------------- SUBFIGURE -5 -------------- %
    \subfigure[real 330us]{
    \includegraphics[width=\width] {./figs/real_out/50}
    \label{fig:r5_out}
  }
    % -------------- SUBFIGURE -6 -------------- %
    \subfigure[real 425us]{
    \includegraphics[width=\width] {./figs/real_out/60}
    \label{fig:r6_out}
  }
  \end{minipage}%
  \begin{minipage}[b]{0.45\textwidth}%
  \centering%
    % -------------- SUBFIGURE -1 -------------- %
    \subfigure[synthetic 50us]{
    \includegraphics[width=\width] {./figs/synth_out/syn1}
    \label{fig:s1_out}
  }
    % -------------- SUBFIGURE -2 -------------- %
    \subfigure[synthetic 95us]{
    \includegraphics[width=\width] {./figs/synth_out/syn10}
    \label{fig:s2_out}
  }
    % -------------- SUBFIGURE -3 -------------- %
    \subfigure[synthetic 140us]{
    \includegraphics[width=\width] {./figs/synth_out/syn20}
    \label{fig:s3_out}
  }
  \\
    % -------------- SUBFIGURE -4 -------------- %
    \subfigure[synthetic 235us]{
    \includegraphics[width=\width] {./figs/synth_out/syn40}
    \label{fig:s4_out}
  }
    % -------------- SUBFIGURE -5 -------------- %
    \subfigure[synthetic 330us]{
    \includegraphics[width=\width] {./figs/synth_out/syn50}
    \label{fig:s5_out}
  }
    % -------------- SUBFIGURE -6 -------------- %
    \subfigure[synthetic 425us]{
    \includegraphics[width=\width] {./figs/synth_out/syn60}
    \label{fig:s6_out}
  }
  \end{minipage}\\
  \begin{minipage}[b]{0.45\textwidth}%
  \centering%
    \subfigure[Optimal (75us)]{
    \includegraphics[width=0.3\textwidth] {./figs/real_out/6}
    \label{fig:opt_real_out}
  }
    \subfigure[EWG]{
    \includegraphics[trim = 100 280 120 280, clip, width=0.3\textwidth]{./figs/realoutdoor_EWG.pdf}% l b r t
    \label{fig:EWG_real_out}
  }
  \end{minipage}
  \begin{minipage}[b]{0.45\textwidth}%
  \centering%
    \subfigure[Optimal (70us)]{
    \includegraphics[width=0.3\textwidth] {./figs/synth_out/syn5}
    \label{fig:opt_synth_out}
  }
    \subfigure[EWG]{
    \includegraphics[trim = 100 280 120 280, clip, width=0.3\textwidth]{./figs/synoutdoor_EWG.pdf}% l b r t
    \label{fig:EWG_synth_out}
  }
  \end{minipage}

  \caption{Experiments in an outdoor environment with an illumination of more than 8000 lux.}

  \label{fig:synth_exp_out}
\end{figure*}


==> fig_synth_gain_indoor.tex <==
\begin{figure*}[tb]
  \centering%
  \def\width{0.25\columnwidth}%
  \begin{minipage}[b]{0.45\textwidth}%
  \centering%
    % -------------- SUBFIGURE -1 -------------- %
    \subfigure[real 0dB ]{
    \includegraphics[width=\width] {./figs/synth_g/25_1}
    \label{fig:25_1}
  }
    % -------------- SUBFIGURE -2 -------------- %
    \subfigure[real 3dB]{
    \includegraphics[width=\width] {./figs/synth_g/25_3}
    \label{fig:25_3}
  }
    % -------------- SUBFIGURE -3 -------------- %
    \subfigure[real 5dB]{
    \includegraphics[width=\width] {./figs/synth_g/25_5}
    \label{fig:25_5}
  }
  \\
    % -------------- SUBFIGURE -4 -------------- %
    \subfigure[real 7dB]{
    \includegraphics[width=\width] {./figs/synth_g/25_7}
    \label{fig:25_7}
  }
    % -------------- SUBFIGURE -5 -------------- %
    \subfigure[real 9dB]{
    \includegraphics[width=\width] {./figs/synth_g/25_9}
    \label{fig:25_9}
  }
    % -------------- SUBFIGURE -6 -------------- %
    \subfigure[real 11dB]{
    \includegraphics[width=\width] {./figs/synth_g/25_11}
    \label{fig:25_11}
  }
  \end{minipage} %
  \begin{minipage}[b]{0.45\textwidth}%
  \centering%
    % -------------- SUBFIGURE -1 -------------- %
    \subfigure[synthetic 0dB]{
    \includegraphics[width=\width] {./figs/synth_g/s1}
    \label{fig:g1}
  }
    % -------------- SUBFIGURE -2 -------------- %
    \subfigure[synthetic 3dB]{
    \includegraphics[width=\width] {./figs/synth_g/s3}
    \label{fig:g3}
  }
    % -------------- SUBFIGURE -3 -------------- %
    \subfigure[synthetic 5dB]{
    \includegraphics[width=\width] {./figs/synth_g/s5}
    \label{fig:g5}
  }
  \\
    % -------------- SUBFIGURE -4 -------------- %
    \subfigure[synthetic 7dB]{
    \includegraphics[width=\width] {./figs/synth_g/s7}
    \label{fig:g7}
  }
    % -------------- SUBFIGURE -5 -------------- %
    \subfigure[synthetic 9dB]{
    \includegraphics[width=\width] {./figs/synth_g/s9}
    \label{fig:g9}
  }
    % -------------- SUBFIGURE -6 -------------- %
    \subfigure[synthetic 11dB]{
    \includegraphics[width=\width] {./figs/synth_g/s11}
    \label{fig:g11}
  }
  \end{minipage}\\
  \begin{minipage}[b]{0.45\textwidth}%
  \centering%
    \subfigure[Optimal (0dB)]{
    \includegraphics[width=0.3\textwidth] {./figs/synth_g/25_1}
    \label{fig:opt_real_g}
  }
    \subfigure[EWG]{
  \includegraphics[trim = 100 280 120 280, clip, width=0.3\textwidth]{./figs/real_gainEWG}% l b r t
    \label{fig:EWG_real_g}
  }
  \end{minipage}
  \begin{minipage}[b]{0.45\textwidth}%
  \centering%
    \subfigure[Optimal (0dB)]{
    \includegraphics[width=0.3\textwidth] {./figs/synth_g/s1}
    \label{fig:opt_synth_g}
  }
    \subfigure[EWG]{
   \includegraphics[trim = 100 280 120 280, clip, width=0.3\textwidth]{./figs/synth_gainEWG}% l b r t
    \label{fig:EWG_synth_g}
  }
  \end{minipage}
  \caption{Comparison of synthetic images and actual images along the gain variation.}

  \label{fig:synth_gain}
\end{figure*}


==> fig_synth_gain_outdoor.tex <==
\begin{figure*}[!t]
  \centering%
  \def\width{0.25\columnwidth}%
  \begin{minipage}[b]{0.49\textwidth}%
  \centering%
    % -------------- SUBFIGURE -1 -------------- %
    \subfigure[real 0dB]{
    \includegraphics[width=\width] {./figs/real_out_g/1}
    \label{fig:r1g_out}
  }
    % -------------- SUBFIGURE -2 -------------- %
    \subfigure[real 2dB]{
    \includegraphics[width=\width] {./figs/real_out_g/3}
    \label{fig:r2g_out}
  }
    % -------------- SUBFIGURE -3 -------------- %
    \subfigure[real 5dB]{
    \includegraphics[width=\width] {./figs/real_out_g/6}
    \label{fig:r3g_out}
  }
  \\
    % -------------- SUBFIGURE -4 -------------- %
    \subfigure[real 8dB]{
    \includegraphics[width=\width] {./figs/real_out_g/9}
    \label{fig:r4g_out}
  }
    % -------------- SUBFIGURE -5 -------------- %
    \subfigure[real 10dB]{
    \includegraphics[width=\width] {./figs/real_out_g/11}
    \label{fig:r5g_out}
  }
    % -------------- SUBFIGURE -6 -------------- %
    \subfigure[real 12dB]{
    \includegraphics[width=\width] {./figs/real_out_g/13}
    \label{fig:r6g_out}
  }
  \end{minipage}%
  \begin{minipage}[b]{0.45\textwidth}%
  \centering%
    % -------------- SUBFIGURE -1 -------------- %
    \subfigure[synthetic 0dB]{
    \includegraphics[width=\width] {./figs/synth_out_g/syn1}
    \label{fig:s1g_out}
  }
    % -------------- SUBFIGURE -2 -------------- %
    \subfigure[synthetic 2dB]{
    \includegraphics[width=\width] {./figs/synth_out_g/syn3}
    \label{fig:s2g_out}
  }
    % -------------- SUBFIGURE -3 -------------- %
    \subfigure[synthetic 5dB]{
    \includegraphics[width=\width] {./figs/synth_out_g/syn6}
    \label{fig:s3g_out}
  }
  \\
    % -------------- SUBFIGURE -4 -------------- %
    \subfigure[synthetic 8dB]{
    \includegraphics[width=\width] {./figs/synth_out_g/syn9}
    \label{fig:s4g_out}
  }
    % -------------- SUBFIGURE -5 -------------- %
    \subfigure[synthetic 10dB]{
    \includegraphics[width=\width] {./figs/synth_out_g/syn11}
    \label{fig:s5g_out}
  }
    % -------------- SUBFIGURE -6 -------------- %
    \subfigure[synthetic 12dB]{
    \includegraphics[width=\width] {./figs/synth_out_g/syn13}
    \label{fig:s6g_out}
  }
  \end{minipage}\\
  \begin{minipage}[b]{0.45\textwidth}%
  \centering%
    \subfigure[Optimal (3dB)]{
    \includegraphics[width=0.3\textwidth] {./figs/real_out_g/4}
    \label{fig:opt_real_out_g}
  }
    \subfigure[EWG]{
    \includegraphics[trim = 100 280 120 280, clip, width=0.3\textwidth]{./figs/real_out_g/real_gain_EWG.pdf}% l b r t
    \label{fig:EWG_real_out_g}
  }
  \end{minipage}
  \begin{minipage}[b]{0.45\textwidth}%
  \centering%
    \subfigure[Optimal (2dB)]{
    \includegraphics[width=0.3\textwidth] {./figs/synth_out_g/syn3}
    \label{fig:opt_synth_out_g}
  }
    \subfigure[EWG]{
    \includegraphics[trim = 100 280 120 280, clip, width=0.3\textwidth]{./figs/synth_out_g/syn_gain_EWG.pdf}% l b r t
    \label{fig:EWG_synth_out_g}
  }
  \end{minipage}

  \caption{Experiments in an outdoor environment with an illumination of more than 8000 lux.}

  \label{fig:synth_exp_out_g}
\end{figure*}


==> tab_dataset.tex <==
%TABLE
\begin{table*}[!h]
  \centering
  \caption{Optimal parameters in each environment}
  \label{tab:data}

  \begin{tabular}{c|ccccccc}
    \textbf{Illuminance {[}lux{]}}  & 10                         & 50                   & 80               & 100               & 320             & 400                & 1000\\
    \hline
    \textbf{environment}            & \textit{Dark surroundings} & \textit{Living room} & \textit{Hallway} & \textit{Dark day} & \textit{Office} & \textit{Sunny day} & \textit{Artificial lighting}\\
    \hline
    \textbf{Optimal $\Delta$t [ms]} & 17.0                       & 20.0                 & 5.5              & 5.5               &   2.5           & 2.0                & 2.0\\
    \hline
    \textbf{Optimal gain [dB]}      & 11                         & 3                    & 0                & 0                 &  12             & 4                  & 1\\
    \hline\hline
    \textbf{Optimal $\Delta$t [ms]} & 19.5                       & 12.5                 & 5.5              & 5.0               &   7.0           & 2.0                & 1.5\\
    \hline
    \textbf{Optimal gain [dB]}      & 9                          & 0                    & 0                & 0                 &  2              & 4                  & 0

  \end{tabular}
\end{table*}
%TABLE

